When simplicity meets effectiveness: Detecting code comments coherence with word embeddings and LSTM

Code comments play a crucial role in software development, as they provide programmers with practical information, allowing them to understand better the intent and semantics of the underpinning code. Nevertheless, developers tend to leave comments unchanged after updating the code, resulting in a discrepancy between the two artifacts. Such a discrepancy may trigger misunderstanding and confusion among developers, impeding various activities, including code comprehension and maintenance. Thus, it is crucial to identify if, given a code snippet, its corresponding comment is coherent and reflects well the intent behind the code. Unfortunately, existing approaches to this problem, while obtaining an encouraging performance, either rely on heavily pre-trained models, or treat input data as text, neglecting the intrinsic features contained in comments and code, including word order and synonyms. This work presents Co3D as a practical approach to the detection of code comment coherence. We pay attention to internal meaning of words and sequential order of words in text while predicting coherence in code-comment pairs. We deployed a combination of Gensim word2vec encoding and a simple recurrent neural network, a combination of Gensim word2vec encoding and an LSTM model, and CodeBERT. The experimental results show that Co3D obtains a promising prediction performance, thus outperforming well-established baselines. We conclude that depending on the context, using a simple architecture can introduce a satisfying prediction.

==> src/Approach.tex <==
The proposed approach


\subsection{CodeBERT}

Something about CodeBERT here.


\begin{figure}[t!]
	\vspace{-.2cm}
	\centering
	\includegraphics[width=0.80\linewidth]{figs/System.pdf}
	\caption{System architecture.}
	\label{fig:System}
	\vspace{-.6cm}
\end{figure}



\begin{table}[h!]
  \begin{center}
    \caption{Your first table.}
    \label{tab:table1}
    \begin{tabular}{l|c|r} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
      \textbf{Value 1} & \textbf{Value 2} & \textbf{Value 3}\\
      $\alpha$ & $\beta$ & $\gamma$ \\
      \hline
      1 & 1110.1 & a\\
      2 & 10.1 & b\\
      3 & 23.113231 & c\\
      4 & something & c\\
    \end{tabular}
  \end{center}
\end{table}


\begin{itemize}
\item The first item.
\item The second item.

\end{itemize}

==> src/Threat.tex <==
There are a couple of threats to the validity of the work, with the most notable being the quality of the dataset. As the saying goes “The model is only as good as the data”, which relates to both data quantity \cite{4804817} and quality, and can be seen from the overall model performance on the JHotDraw741 dataset. This particular dataset was one with lowest Kappa index, with its weighted Kappa index being below 0.70 \cite{DBLP:conf/clic-it/CorazzaMS16} which can be seen reflecting across all models experimented with. Therefore, the quality of the dataset used in this paper could be a threat to the validity of the work.

Another notable threat is the amount of information discarded during the text encoding section of the research. Due to the large processing time needed to encode all the dataset for training, each code-comment pair was truncated or padded to the first 50 vectors corresponding to the first 50 word/symbols from each code-comment pair (for the SimpleRNN and LSTM pairs). This can be seen as a lot of information discarded considering that the longest code-comment pair had a word/symbol length above 500. Similarly for the BERT and CodeBERT (although less extreme), each entry was truncated to average length of 113 which is still significantly smaller compared to the max recorded length above 500, and the maximum allowable length of both models being above 700 tokens. It is possible that with a more distributed and parallel approach to this encoding process in further research and increasing size of the SimpleRNN and LSTM models to account for this increased information, the models might produce better predictions than they already have.

Another possible threat which was also stated in the original paper \cite{DBLP:journals/sqj/CorazzaMS18} is the possibility of bias to the only language used in this paper. Only the Java programming language was used in the construction of the dataset used for this paper, therefore, it isn’t easy to know if the results obtained are specific to this programming language or if it will generalize to other languages. As we have already seen from this paper, the corpus (which can be language specific) does seem to play a role in model performance, hence can also be considered a threat to the work.

Lastly, a more generic threat to this paper is the size of the dataset. More data is almost always considered better \cite{4804817}, and a total of 5762 entries is arguably small for the size of models they were trained on, which can lead to overfitting in model performance. 

